PREVis: Perceived Readability Evaluation for Visualizations

We developed and validated an instrument to measure the perceived readability in data visualization: PREVis. Researchers and practitioners can easily use this instrument as part of their evaluations to compare the perceived readability of different visual data representations. Our instrument can complement results from controlled experiments on user task performance or provide additional data during in-depth qualitative work such as design iterations when developing a new technique. Although readability is recognized as an essential quality of data visualizations, so far there has not been a unified definition of the construct in the context of visual representations. As a result, researchers often lack guidance for determining how to ask people to rate their perceived readability of a visualization. To address this issue, we engaged in a rigorous process to develop the first validated instrument targeted at the subjective readability of visual data representations. Our final instrument consists of 11 items across 4 dimensions: understandability, layout clarity, readability of data values, and readability of data patterns. We provide the questionnaire as a document with implementation guidelines on osf.io/9cg8j. Beyond this instrument, we contribute a discussion of how researchers have previously assessed visualization readability, and an analysis of the factors underlying perceived readability in visual data representations.

==> sections/08_conclusion.tex <==
\SkipTocEntry\section{Conclusion}

We developed and validated \scalename, a reliable instrument for measuring perceived readability in data visualization. Researchers can use it to ask participants in empirical studies to rate visualization images, and collect a set of four measures representing the following dimensions we uncovered in this work: \SUn, \SLa, \SDR, and \SDF. At this stage of our research on the topic, we define readability as a product of the interaction between the visual properties of a representation, the cognitive abilities of its reader, and the task context.
\scalename provides multiple opportunities for further research, as discussed in the previous section, which can ultimately contribute to better explain factors and outcomes of readability in data visualization.


==> sections/ZZ_removed_elements.tex <==
\section{Dropped from last introduction}

Researchers have, in the past, collected qualitative measures of how readable study participants find a data visualization to help them refine empirical findings about user experience \cite{ajani_2022_DeclutterFocus}, system usability \cite{baumgartl_2021_SearchPatient}, or insight generation processes \cite{burns_2022_DesigningPictographs}. 
%Collecting qualitative measures of how readable study participants find a data visualization helps researchers to refine \afcs{and explain} empirical findings about user experience, system usability, or insight generation processes. 
In fact, during the preliminary phase of this project we found 34 publications by authors who had asked study participants to rate visualizations with questions related to readability. We also found that these questions varied greatly in terms of wording and answer options. Such discrepancies pose issues of comparability and reliability of empirical findings.
Our \scalename tool addresses this problem because we followed well-established methodologies in scale development \cite{Devellis:2021:ScaleDevelopment, Boateng:2018:BestPractices}. A psychological scale is a study instrument, often in the form of a series of Likert items, that targets a specific construct---in our case, perceived readability in data visualization.
Developing a valid scale requires researchers to review existing literature and collect suggestions of experts on how to phrase the scale's items. In that way, it has been an enriching endeavor that allowed us to better understand the concept of readability in data visualization. %because it required to better understand how the visualization literature has so far talked about the concept, how researchers have studied it, and how experts currently think of it.



\section{Introduction - PETRA'S VERSION}

When looking at examples of data visualizations, it is intuitively clear that some are \afc{easier to read}{}%more readable
than others or, put differently: it seems \afc{simpler}{}%easier
to retrieve information from some \afc{visual representations}{} %visualizations
compared to others. For many data analysis use cases, the readability of shown visualizations is a fundamental quality criterion \cite{Kosara:2007:VisualizationCriticism}.
As such, improving the readability of data visualizations is one of the central research goals in our field and has been addressed by empirical research in many different formats, \eg, basic perceptual studies aimed to explain how viewers perceive a visualization, studies that compare user performance with different visualizations across tasks, or qualitative research aimed at understanding subjective reactions to a visualization design.

One of the fundamental challenges in studying the readability of data visualizations, however, is that the concepts of \emph{reading} and \emph{readability} are held as tacit knowledge.
The terms are often used in writing and user evaluation without clear definitions of what they specifically mean in the context of data visualization---recalling Kosara's ``empire built on sand'' \cite{Kosara:2016}.
Without a formal definition of the factors involved in making visualizations easy or difficult to read, %appear to be more readable than others,
it is unclear to what extent different approaches to measuring readability even target the concept.
To make matters worse, current models of visualization \afc{comprehension}{} \cite{Hegarty:2011:CogVisualRepresentations, Padilla:2018:decision_model, Fox:2023:theories_models} do not %clearly define 
\afc{specify}{}the boundaries of ``reading'' as an activity in which a user engages.
%The models fall short in situating
\afc{While the models provide important theoretical grounding to explain how people process information from data visualizations, they do not situate}{}the reading %process
activity within the \afc{cognition continuum ranging from}{}%continuum of cognitive processes comprising
low-level visual perception \cite{Quadri:2022} to %and
high-level activities such as data exploration \cite{Yalcin:2016}, insight and knowledge generation \cite{Stasko:2014:value-driven-vis, Sacha:2014:Knowledge}, sense-making of unfamiliar visualizations \cite{Lee:2015:sensemaking}, or decision-making \cite{Padilla:2018:decision_model}.

Our work is based on the fundamental premise that the readability of a data visualization is a crucially important quality criterion that requires formal definition and empirically verified methods to study it.  In this paper we present our work on developing a validated scale to measure the perceived readability of visualizations. To do so, we also had to take first steps in clarifying what readability means in data visualization. While we do not promise to entirely define readability---yet---, we posit that %readability
it is not only a characteristic of the visualization; it is also highly individual and situational. As such, in our work, we talk about the concept of \emph{perceived readability} to emphasize that readability is not only a measurable characteristic of the data visualizations---for example, the number of edge crossings in a node-link graph. 

\begin{figure*} [!h]
    \centering
    \includegraphics[width=\textwidth]{figures/Readability_scale_paper_Model_re2.pdf}
    \caption{Our proposition to define the boundaries of \emph{reading} within the model proposed by Hegarty \cite{Hegarty:2011:CogVisualRepresentations}, summarizing Shah \cite{Shah:2005:ComprehensionQuantitativeInformation} and Pinker \cite{Pinker:1990:GraphComprehension}}
    \label{fig:model-reading}
\end{figure*}

A validated scale in psychology is a study instrument, %often in the form of a questionnaire, 
often in the form of a \afc{series of Likert items,}{}that targets a specific construct\afc{---in our case, perceived readability in data visualization.}{}%The construct in our case is perceived readability.
Developing a validated scale has been an enriching endeavor because it required to better understand how the visualization literature has so far talked about the concept, how researchers have studied it, and how experts currently think of it. Our scale can be used in experiments, after participants completed reading tasks, to measure their perception of a data visualization’s readability in a standardized way. In doing so we do not mean to replace other ways of empirical research on data visualizations. Instead, our scale can be used in combination with other
approaches, to help researchers to refine empirical findings about user experience, system usability, or insight generation processes. 

In summary, with our work we make the following contributions:
\begin{itemize}[nosep,left=0pt .. \parindent]
\item a validated scale to study perceived visualization readability that can be deployed in empirical research on data visualization,
\item an analysis of the factors underlying perceived readability of visual data representations, and
\item an in-depth discussion and analysis of the concept of readability and how it has been used in the visualization field.
\end{itemize}
%Ultimately, readability defines how useful or usable a visualization will be to a particular viewer. 




\section{Introduction - AF 1st VERSION}

%What I dislike about the current version is that I come away from the abstract thinking this paper will be completely focused on scale development. The introduction, however, is entirely on reading as a cognitive ability and talks about defining cognitive models, etc. That's not a very good fit. In this alternative I change this by shuffling things around and first talking about readability as an important quality criterion of visualizations. I will steal some text from the ANR project I wrote yesterday

\label{sec:intro}

%2024-01-25:
As external cognition tools, visualizations leverage our brains' high-band\-width visual channel to access encoded data \cite{Munzner:2014,Card:1999}. The visualization research community has long been investigating people's cognitive processes when they engage with data visualizations \cite{Bertin:1983,Cleveland:1984:GraphPerception,Kosslyn:1989:UnderstandingCharts,Pinker:1990:GraphComprehension}.Yet, there is still a knowledge gap regarding how these processes are integrated across levels of cognition \cite{Padilla:2018:Case_cog_models}, and there is a lack of tools for a multi-level evaluation of visual data representations \cite{Kurzhals:2014:EyeTrackingVisAnalytics}.

In particular,  \hty{reading is an important one of these processes[cite \cite{Curcio:1987:MathRelationships}].} The concepts of \emph{reading} and \emph{readability}\hty{, however,} are held as tacit knowledge and that are usually used without clear definitions of what they specifically mean in the context of data visualization.
%, and still under-specified in the context of data visualization.
\hty{Current models of visualization comprehension do not clearly define the boundaries of ``reading'' and  fall short in situating the reading process within the continuum of cognitive processes, ranging from} 
% Cognitive processes are tightly linked %from Quadri & Rosen 2022
% and, thus, difficult to untangle---yet current visualization comprehension models \cite{Fox:2023:theories_models} do not define either the boundaries of what \emph{reading} is. It is also unclear how reading processes fit between 
low-level visual perception \cite{Quadri:2022} and high-level activities such as data exploration \cite{Yalcin:2016}, insight and knowledge generation \cite{Stasko:2014:value-driven-vis, Sacha:2014:Knowledge}, sense-making of unfamiliar visualizations \cite{Lee:2015:sensemaking}, or decision-making \cite{Padilla:2018:decision_model}. To answer calls for the development of cognitive models within visualization %in the data visualization field 
\cite{Padilla:2018:Case_cog_models, Kosara:2016} and for a comprehensive theory of human information processing in visual analytics \cite{Pohl:2012:UserPuzzle}, we thus set out to define the concepts at hand as an important step in this direction.

Among them \hty{(Tingying: What does ``them'' refer to?)}, \emph{readability} is regarded as an essential quality for data visualization. Yet, because meaning is constructed by the reader \cite{Fox:2023:Vis_Psych_foundations}, readability is not only a characteristic of the visual image---it is also highly individual and situational. %« the relation between the “thing” and the “representation” is not a direct and determined mapping, but entirely subjective, based on the interpretation of the observer. \cite{Fox:2023:Vis_Psych_foundations}»
\hty{(Tingying: It would be better if we can refer to any work saying that readability is both subjective and objective?)}
%\afc{
Ultimately, readability defines how useful or usable a visualization will be to a viewer. Being able to establish the readability of a visualization formally is, therefore, of crucial importance to be able to verify and improve visualization recommender tools and to develop onboarding systems that help novice users to read visualizations and understand data. It is also an important measure for testing the scalability and usability of existing visualization techniques and algorithms across different dataset sizes. To be able to reach these goals we thus need to conduct fundamental research on this concept  %of visualization readability, to model it, % TI: I took this part out since we do not really model it, that would be way too much
and to derive validated measures for studying it.%}{from ANR proposal--by Petra I think} 

Such subjective evaluations of readability have the potential to help us ground our understanding of how people process information from visual representations within the visualization psychology framework \cite{Fox:2023:Vis_Psych_foundations}---yet we lack \emph{standardized} instruments to measure it.
% We consider that a better understanding of readability’s factors and effects would help in improving theoretical models of visualization comprehension (and of resulting higher-level cognitive activities such as decision-making); and in refining and possibly expanding visualization design frameworks.
%To achieve such goals, we need validated measuring instruments.
We thus developed and validated a psychological scale to measure the perceived readability of visualizations, to take a first step towards clarifying what readability means in data visualization. Our scale can be used in experiments, after participants completed reading tasks, to measure their perception of a data visualization's readability in a standardized way. In doing so we do not mean to replace other measures of technique performance. Instead, our scale can be used in combination with other measures, to help researchers to %explain collected information
refine empirical findings about user experience, system usability, or insight generation processes.







% - We generate a pool of candidate items from deductive and inductive methods
% - After a qualitative pre-test study, we conduct an Exploratory Factor Analysis on data collected through a crowd-sourced survey and identify x dimensions of the construct
% - We filter items down and conduct dimensionality, reliability and validity tests on the final scale





==> tables/items_generation_revisions.tex <==
\begin{table*}[t]
\centering
\footnotesize
\tabulinesep=0.8mm
\caption{39 items generated from primary and secondary relevant terms.}
\label{tab:items_generation_revisions}
\begin{tabu} to \textwidth{X[2] X[0.5] X[1] X[2]}
\toprule
Item statement (reviewed) & Root stems & Secondary stems & Item statement (initial version)\\ 
\midrule
I can answer questions about the data after reading this visualization & answer & data, read & After reading this visualization, I could answer questions about the data\\ 
The visual encodings (e.g., color, shapes...) in this visualization make the information clear to me & clear & encod, inform & The visual encodings (e.g., color, shapes...) make the information clear\\ 
This visualization shows information in a clear way for me & clear & inform & This visualization shows (relevant/key) information in a clear way\\ 
I find this visualization cluttered [reverted item] & clutter &  - & [Reverted] This visualization is cluttered\\ 
I find this visualization complex to read [reverted item] & complex & read & [Reverted] The visualization is too complex\\ 
I am confident in my interpretation of this visualization & confid & interpret & I am confident in my interpretation of this visualization\\ 
I find this visualization confusing [reverted item] & confus &  - & [Reverted] This visualization is confusing\\ 
This visualization allows me to correctly interpret the data & correct & data & This visualization allows me to correctly interpret the data\\ 
I find the visual encodings (e.g., color, shapes...) difficult to decipher in this visualization [reverted item] & deciph & difficult, encod & [Reverted] The visual encodings are difficult to decipher\\ 
I can determine key information in this visualization & determin & key, inform & I can determine key information in this visualization\\ 
This visualization allows me to discern elements of the data & discern & data & This visualization allows me to discern elements of the data\\ 
I find parts of the visualization distracting [reverted item] & distract &  - & Some parts of the visualization are distracting\\ 
This visualization effectively shows the data to me & effect & data, show & This visualization effectively shows the data\\ 
I can understand how the data is encoded in this visualization & encod & data, understand & I understand how the data is encoded in this visualization\\ 
I can easily find specific elements or information in this visualization & find & easili, inform & It is easy to find specific elements or information in this visualization\\ 
I find this visualization easy to follow & follow & easi & This visualization is easy to follow\\ 
This visualization helps me understand the data & help & understand, data & This visualization helps me understand the data\\ 
I can identify relevant information in this visualization & identifi & relev, inform & I can identify relevant information in this visualization\\ 
I can easily retrieve information from this visualization & inform & easili & I can easily retrieve information from this visualization\\ 
I find this visualization informative & inform &  - & This visualization is informative\\ 
I find this visualization easy to interpret & interpret & easi & This visualization is easy to interpret\\ 
I find this visual design intuitive & intuit & visual, design & This visual design is intuitive\\ 
The visual encodings (e.g., color, shapes) in this visualization make sense to me & make sense & encod
("make sense" is used as a replacement for "meaningful") & The visual encodings (e.g., color, shapes...) are appropriate in this visualization\\ 
I can easily interpret the overall meaning of the data visualization & mean & overall, interpret & I can easily interpret the overall meaning of the data visualization\\ 
I can understand what the visual components of the visualization mean & mean & understand, visual, compon & I understand what the visual components of the visualization mean\\ 
It is obvious for me how to read this visualization & obvious & read & It is obvious how to read this visualization\\ 
I find this visualization well organized & organiz & ("organiz" is used as a replacement for "arrang") & This visualization is well organized\\ 
This visualization provides me with a good overview of the data & overview & data & This visualization provides a good overview of the data\\ 
I can easily perceive data features (e.g., trends, minimums, outliers...) in this visualization & perceiv & easili, data, featur & It is easy to perceive data features in this visualization\\ 
I can easily read this visualization & read & easili & I can easily read this visualization\\ 
I find this visualization readable & readabl &  - & This visualization is readable\\ 
I can recognize data features (e.g., trends, minimums, outliers...) in this visualization & recogn & data, featur & I can recognize features of the data (e.g., trends, patterns...) in this visualization\\ 
I can clearly see data features (e.g., trends, minimums, outliers...) in this visualization & see & data, featur, clear & I can clearly see data features in this visualization\\ 
This visualization shows the data in an appropriate manner for me & show & data & This visualization shows the data in an appropriate manner\\ 
I find this visualization simple to read & simpl & read & This visualization is simple\\ 
I can easily understand this visualization & understand & easili & I can easily understand this visualization\\ 
I can quickly understand this visualization & understand & quick & I can quickly understand this visualization\\ 
I can extract data values from this visualization & valu & data & I can extract data values from this visualization\\ 
I find data features (e.g., trends, minimums, outliers...) visible in this visualization & visibl & featur & The data features are visible in this visualization\\ 
\bottomrule
\end{tabu}
\end{table*}

==> tables/parallel_analyses.tex <==
\begin{table}[h!]
\centering
%\footnotesize
\fontsize{7pt}{7pt}\selectfont
\caption{Survey-wise and stimulus-wise number of factors as output from parallel analysis.}
\label{tab:parallel_analyses}
\tabulinesep=0.8mm
\begin{tabu} to \linewidth {X[1,l]X[1,l]}
\toprule Dataset & Suggested number of factors from Parallel Analysis \\
\midrule

Full survey & 5 \\
Stimulus A & 5 \\
Stimulus B &  4 \\
Stimulus C & 3 \\
Stimulus D & 4 \\
Stimulus E & 4 \\
Stimulus F & 3 \\
\bottomrule
\end{tabu}
\end{table}
